Millimeter-Wave UAV Coverage in Urban Environments

With growing interest in mmWave connectivity for UAVs, a basic question is whether networks intended for terrestrial users can provide sufficient aerial coverage as well. To assess this possibility, the paper proposes a novel evaluation methodology using generative models trained on detailed ray tracing data. These models capture complex propagation characteristics and can be readily combined with antenna and beamforming assumptions. Extensive simulation using these models indicate that standard (street-level and downtilted) base stations at typical microcellular densities can indeed provide satisfactory UAV coverage. Interestingly, the coverage is possible via a conjunction of antenna sidelobes and strong reflections. With sparser deployments, the coverage is only guaranteed at progressively higher altitudes. Additional dedicated (rooftop-mounted and uptilted) base stations strengthen the coverage provided that their density is comparable to that of the standard deployment, and would be instrumental for sparse deployments of the latter.

==> extra.tex <==


 %Minimum distance is set to $10$m for BSs and UAVs respectively. The affect of noise is considered by a noise figure of $6$ dB over channel bandwidth of $400$ MHz.
Consider the channel connecting the $i$th UAV with the $j$th gNB.
Given the distance and direction and between the UAV and gNB, the neural network
generates a random set of paths.  Each path has a direction 
Given the elevation and azimuth angles-of-arrival (AOA) at the receiver for the $\ell$th connecting path, ($\theta_{i,j,\ell}^{\sf rx}, \phi_{i,j,\ell}^{\sf rx}$), and the corresponding angles-of-departure (AOD) at the transmitter, ($\theta_{i,j,\ell}^{\sf tx}, \phi_{i,j,\ell}^{\sf tx}$), the matrix for that channel is
\begin{equation}
\begin{split}
\label{eq:channel}
    \bH_{i,j} = \sum_{\ell=1}^{L} g_{i,j,l}(\theta_{i,j,\ell}^{\sf rx},\phi_{i,j,\ell}^{\sf rx},\theta_{i,j,\ell}^{\sf tx},\phi_{i,j,\ell}^{\sf tx}) \\ 
 \bu (\theta_{i,j,\ell}^{\sf rx}, \phi_{i,j,\ell}^{\sf rx} ) \, \bv^* (\theta_{i,j,\ell}^{\sf tx}, \phi_{i,j,\ell}^{\sf tx} ),
\end{split}
\end{equation}
where $L$ is the number of paths, $g_{i,j,\ell}(\cdot)$ subsumes the pathloss for the $\ell$th path and the appropriate element antenna gains at both receiver and transmitter, and $\bu(\cdot)$ and $\bv(\cdot)$ are the array response vectors at receiver and transmitter. Beamforming is applied towards the strongest path, yielding a beamforming gain of
\begin{equation}
\label{eq:G_b}
    G_{i,j} = \big| \bw^*_{j} \bH_{i j} \bff_i \big|^{2}
\end{equation}
where $\bw_j=\bu(\theta_{i,j,k}^{\sf rx}, \phi_{i,j,k}^{\sf rx} )$ and $\bff_i=\bv(\theta_{i,j,k}^{\sf rx}, \phi_{i,j,k}^{\sf rx})$ are the beamforming vectors at receiver and transmitter with $k$ the index of that strongest path \cite[sec. 3.5]{heath2018foundations}.
The signal-to-noise ratio (SNR) between UAV $i$ and gNB $j$ is then
\begin{equation}
\label{eq:SNR}
    \SNR_{i,j} = \frac{P~G_{i,j}}{N_{0} B},
\end{equation}
where $P$ is the UAV transmit power and $N_0 B$ is the noise power over bandwdith $B$. Each UAV connects to the gNB to which it has the highest SNR.

%A large-scale simulation campaign is conducted by iteratively dropping UAVs and BSs with all the settings over the network area.

%\begin{itemize}[leftmargin=*]
   % \item \emph{Area:} 1000 m $\times$ 1000 m.
%    \item \emph{Distribution of Terrestrial gNBs:} The deployment follows a Poisson Point Process (PPP) that matches an inter-site distance (ISD) equal to 200 m, and a minimum distance between each pair of terrestrial gNBs equal to 10 m.
%    \item \emph{Height of Terrestrial gNBs:} Uniformly distributed between 2 m and 5 m.
%    \item \emph{Distribution of Aerial gNBs:} PPP matching the following ISD values: 400 m, 200 m, and 100m. Similarly, we enforce a minimum distance between each pair of aerial gNBs equal to 10 m.
%    \item \emph{Height of Aerial gNBs:} Uniformly distributed between 30 m and 60 m.
%    \item \emph{UAVs:} 1000 uniformly distributed UAVs at three different heights: 30 m, 60 m and 120 m.
%    \item \emph{Association policy:} We pick the link with best SNR after beamforming.
%\end{itemize}



looks at the three
regions of the SNR distribution: a lower tail, middle, and upper tail.  For the UAVs at 
\SI{30}{m} altitude, the divisions between the 
SNR sections were selected at 20 and 95\%. For \SI{120}{m} altitude, the divisions were at
10 and 60\%.  For each section, we compute the fraction of links that are (i) NLOS (meaning no LOS paths), (ii) dominant LOS (meaning there is a LOS path and it is the strongest path),
(iii) LOS with dominant NLOS (meaning there is an LOS path, but an NLOS path is dominant).



==> future_work.tex <==
\section{Future work}
\label{sec:fut}

In this paper, we have discussed the coverage of UAVs in terms of SNR from their serving gNBs. We only considered SNR values for each link between UAVs and gNBs, adding dedicated gNBs. However, we didn't consider interference impact for every connection of UAVs. While UAVs have good link quality, they can suffer from interference caused by nearby moving UAVs or gNBs. In such case, we have to reconsider the coverage of gNBs when UAVs move around and cause interference to others. Thus, in future work, we will take into account the case where UAVs move around and get connections with GNBs and analyze the single to interference ratio (SINR), which reflect more realistic situations of UAV communication. 
